The Busemann Process and Steep Highways in Directed First Passage Percolation

We consider the Busemann process in planar directed first passage percolation. We extend existing techniques to establish the existence of the process in our setting and determine its distribution in a number of integrable models. As examples of their utility, we show how these explicit distributions may be used to quantify the semi-infinite geodesics passing through thin rectangles, and the clustering phenomenon observed in competition interface angles. There is a natural connection with various particle systems, and in particular we obtain the multi-class invariant distributions for discrete-time TASEP with parallel updates.

==> preamble.tex <==
% Updated 2025-08-15

\RequirePackage[l2tabu,orthodox]{nag}  % force newer (and safer) LaTeX commands
\RequirePackage[utf8]{inputenc}

\RequirePackage[a4paper]{geometry}
\RequirePackage{microtype}

\RequirePackage{caption, subcaption}

\RequirePackage{mathtools, amssymb, amsthm, thmtools}

\RequirePackage{booktabs, array}

\RequirePackage{appendix}

\RequirePackage{datetime}
\newdateformat{usvardate}{%
	\THEDAY\  \monthname[\THEMONTH] \THEYEAR}
\usvardate


% Fonts
\RequirePackage{amsfonts, mathrsfs, bbm}

\RequirePackage{enumitem}

\RequirePackage{color}

% tikz
\RequirePackage{tikz}
\usetikzlibrary {positioning} 
\usetikzlibrary{arrows.meta}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.pathmorphing}

% Bibliography
\RequirePackage[backend=biber,style=alphabetic]{biblatex}
\bibliography{biblio.bib}

% Auxiliary commands
\RequirePackage{xspace}
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}

% Operators. Usage: \GL
\def\oper#1{\csdmat{#1}{\operatorname{#1}}}
\forcsvlist\oper{GL,SL,deg,Spec,Hom,End,Vect,Mod,Rep,Ker,Im,Id,Aut,lcm, dist, diam, tr, ker, im, Sym, Span, Res, sinc, supp, Arg, var}
\DeclareMathOperator{\RE}{Re}
\DeclareMathOperator{\IM}{Im}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

% Mathbb Letters. Usage: \bA
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\forcsvlist\defbb{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

% Structures
\def\eq#1{\begin{equation}#1\end{equation}}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2

\def\conj#1{\overline{#1}}
\newcommand{\pder}[2][]{\frac{\partial#1}{\partial#2}}
\newcommand{\mpder}[3][]{\frac{\partial^{#3}#1}{\partial#2^{#3}}}

% Delimiters
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\brac{\lparen}{\rparen}
\DeclarePairedDelimiter\sqrbrac{[}{]}
\DeclarePairedDelimiter\inner{\langle}{\rangle}
\DeclarePairedDelimiter\set{\{}{\}}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

% Extended delimiters
\DeclarePairedDelimiterXPP\Ex[1]{\mathbb{E}}[]{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Exsub[2]{\mathbb{E}_{#2}}[]{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Exabs[1]{\mathbb{E}}\lvert\rvert{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Prob[1]{\mathbb{P}}(){}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Probsub[2]{\mathbb{P}_{#2}}(){}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Var[1]{\mathrm{Var}}\lparen\rparen{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Cov[1]{\mathrm{Cov}}\lparen\rparen{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Corr[1]{\mathrm{Corr}}\lparen\rparen{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}

% Distributions
\newcommand{\Exp}{\ensuremath{\mathrm{Exp}}}
\newcommand{\Ber}{\ensuremath{\mathrm{Ber}}}
\newcommand{\Geom}{\ensuremath{\mathrm{Geom}}}
\newcommand{\Unif}{\ensuremath{\mathrm{Unif}}}

% Shorthands
\newcommand{\disteq}{\ensuremath{\stackrel{d}{=}}}
\newcommand{\given}{\ensuremath{\mid}}
\newcommand{\mto}{\ensuremath{\mapsto}}
\newcommand{\bone}{\mathbbm{1}}

% Wide accents
\DeclareFontFamily{U}{mathx}{}
\DeclareFontShape{U}{mathx}{m}{n}{<-> mathx10}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareMathAccent{\widehat}{0}{mathx}{"70}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}

% Independece symbols
\RequirePackage{rotating,centernot,cancel}    %% to manipulate symbols 
\def\indep{\ \ \;{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\models$\end{rotate}}}}\ \, }  %independent random variables 
\def\nindep{\ \ \,{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\nvDash$\end{rotate}}}}\ \, }   %not independent random variables 

% Bolded item numbers
\newcommand{\bitem}[1]{\item[\textbf{#1.}]}

% Mathbb Letters. Usage: \bA
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\forcsvlist\defbb{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

% Mathcal Letters. Usage: \cA
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\forcsvlist\defcal{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

% Script Letters. Usage: \sA
\def\defscr#1{\csdmat{scr#1}{\mathscr{#1}}}
\forcsvlist\defscr{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z,a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

% Fraktur Letters. Usage: \fkA
\def\deffrak#1{\csdmat{frak#1}{\mathfrak{#1}}}
\forcsvlist\deffrak{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z,a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

% Almost everywhere abbreviations
\newcommand{\es}{\ensuremath{\ \mathrm{a.s}}}
\newcommand{\as}{\ensuremath{\ \mathrm{a.s}}}
\newcommand{\io}{\ensuremath{\ \mathrm{i.o}}}
\newcommand{\fo}{\ensuremath{\ \mathrm{f.o}}}

% Macro for nicer restriction spacing

\newcommand{\littletaller}{\mathchoice{\vphantom{\big|}}{}{}{}}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \littletaller % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

\RequirePackage[colorlinks,urlcolor=blue,linkcolor=red,citecolor=green, hypertexnames=false]{hyperref}
\RequirePackage[capitalize]{cleveref}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{claim}{Claim}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}

% Lists inside theorems (for cleverref)
\newlist{thmlist}{enumerate}{1}
\setlist[thmlist]{label=(\roman{thmlisti}), ref=\thetheorem.(\roman{thmlisti})}
\crefname{thmlisti}{theorem}{theorems}
\crefname{proplisti}{proposition}{propositions}

\newlist{proplist}{enumerate}{1}
\setlist[proplist]{label=(\roman{proplisti}), ref=\thetheorem.(\roman{proplisti})}
\crefname{prop}{proposition}{propositions}

\newlist{corlist}{enumerate}{1}
\setlist[corlist]{label=(\roman{corlisti}), ref=\thetheorem.(\roman{corlisti})}
\crefname{cor}{corollary}{Corollaries}

\Crefname{thm}{Theorem}{Theorems}
\Crefname{lem}{Lemma}{Lemmas}
\Crefname{app}{Appendix}{Appendices}
\Crefname{prop}{Proposition}{Propositions}
